Semantic Compression With Large Language Models

The rise of large language models (LLMs) is revolutionizing information retrieval, question answering, summarization, and code generation tasks. However, in addition to confidently presenting factually inaccurate information at times (known as "hallucinations"), LLMs are also inherently limited by the number of input and output tokens that can be processed at once, making them potentially less effective on tasks that require processing a large set or continuous stream of information. A common approach to reducing the size of data is through lossless or lossy compression. Yet, in some cases it may not be strictly necessary to perfectly recover every detail from the original data, as long as a requisite level of semantic precision or intent is conveyed. This paper presents three contributions to research on LLMs. First, we present the results from experiments exploring the viability of approximate compression using LLMs, focusing specifically on GPT-3.5 and GPT-4 via ChatGPT interfaces. Second, we investigate and quantify the capability of LLMs to compress text and code, as well as to recall and manipulate compressed representations of prompts. Third, we present two novel metrics -- Exact Reconstructive Effectiveness (ERE) and Semantic Reconstruction Effectiveness (SRE) -- that quantify the level of preserved intent between text compressed and decompressed by the LLMs we studied. Our initial results indicate that GPT-4 can effectively compress and reconstruct text while preserving the semantic essence of the original text, providing a path to leverage $\sim$5$\times$ more tokens than present limits allow.

==> sections/contributions.tex <==
\section{Contributions}
\label{contributions}

This paper presents an initial study of compression in Large language models (LLMs) and proposes novel metrics for evaluating the effectiveness of such compression techniques. The main contributions of this work can be divided into two major subsections: the analysis of LLM compression, and the development of the Semantical Compression Metric and Exact Compression Metric.

\subsection{Analysis of LLM Compression}
The analysis of LLM compression is an important aspect of this paper. We thoroughly examined various methods for compressing the text output of LLMs, enabling these models to generate and understand code more efficiently. Our investigation reveals that LLMs can maintain a high level of performance while generating code from compressed text descriptions. This is crucial for academia and research, as it has the potential to improve the efficiency and scalability of LLMs in a wide range of applications.

Moreover, our study demonstrates that LLMs can reconstruct code accurately in a variety of situations when provided with compressed text descriptions. This finding has profound implications for the development of new, more efficient LLM architectures and their deployment in real-world use cases. The ability to decrease the prompt size needed for code generation and understanding can lead to exponentially larger throughput for LLM models, making them more viable for large-scale tasks.

\subsection{Proposed Semantical Compression Metric and Exact Compression Metric}
The development of the Semantical Compression Metric and Exact Compression Metric is another significant contribution of this paper. These metrics provide a rigorous, quantifiable method for evaluating the effectiveness of LLM compression techniques. By offering a standardized means of assessment, our proposed metrics can facilitate further research on LLM compression and contribute to the development of better-performing, more efficient models.

The Semantical Compression Metric measures the preservation of meaning in compressed text, while the Exact Compression Metric quantifies the loss of exact text information. Together, these metrics offer a comprehensive evaluation of LLM compression performance, considering both the semantic aspects and the precise textual content. This is crucial for both academia and research, as it allows for a more nuanced understanding of the trade-offs and benefits associated with different compression techniques.

In summary, our work provides valuable insights into the current state of LLM compression and proposes new metrics for evaluating the performance of these techniques. The findings presented in this paper have broad implications for academia and research, offering a foundation for future studies and the development of more efficient, effective LLMs.

==> sections/future.tex <==
\section{Future Directions}
\label{future_research}


The following is a non-comprehensive summary of questions that may be of interest for future work in the area of approximate compression with LLMs:
%broad areas and suggested directions that we would like to address in future work.

\begin{enumerate}
    \item {For how long of an inference period can recalled compressed text persist? } 

    % The persistence of compression across an inference period depends on the model architecture, compression techniques employed, and the complexity of the information being compressed. Longer inference periods may result in information degradation, but novel approaches to LLM-based compression could improve the stability and persistence of compressed data, opening up new possibilities for efficient long-term information storage and retrieval.
    % \\

    \item {What meta-representations (e.g., unicode, emoji, math symbols, etc.) are LLMs biased towards, if any? Similarly, what is the derived relative information density of each meta-representation when used by an LLM?} 

    %  and how robust are they between inference periods? 

    % LLM biases towards certain meta-representations may stem from the nature of their training data. Although biases may exist, it is crucial to evaluate the robustness of these meta-representations between inference periods and to quantify their relative information density. Identifying these biases and characterizing their impact on LLM performance can inform the development of more balanced and effective compression techniques.
    % \\
    
    \item {What is the minimal prompt that achieves a compression rate of X for a specific type of data?} 

    % Determining the minimal prompt that achieves a specific compression rate requires an understanding of the interplay between the LLM's architecture, the compression algorithm, and the type of data being compressed. Identifying this minimal prompt can improve the efficiency of information transmission and storage, enabling more effective communication and collaboration between LLMs.
    % \\

    \item {How can cooperating/competing LLMs collectively leverage or refine a contextual compression policy?}

    % Cooperating or adversarial LLMs can leverage and improve contextual compression policies by exchanging compressed data, learning from each other's experiences, and identifying weaknesses in the compression process. By doing so, they can enhance the effectiveness and robustness of compression techniques, enabling more efficient information storage and retrieval in a variety of contexts.
    % \\
    
    \item {Can compressed data be embedded into an existing LLM system in an adversarial way to produce undesired behavior?}

    % Compressed text has the potential to be embedded into existing systems as part of adversarial attacks. This highlights the importance of developing robust security measures and data handling protocols to protect against such attacks and to ensure the integrity and privacy of sensitive information.
    % \\

    
    \item {Can approximate compression policies be effectively shared or communicated across models?}

    % Compression can be effectively shared across models, enabling them to benefit from each other's experiences and knowledge. This collaborative approach can lead to more efficient and effective compression techniques, as well as improved generalization and adaptability to different tasks and domains.
    % \\

    \item {Can different contextual categories (e.g., code, prose) be derived to taxonomize LLM compression capabilities?}

    % Contextual categories can be derived to classify LLM compression performance and ability, providing insight into how different models excel in specific tasks or domains. Such categorization can inform model selection, optimization, and deployment strategies, leading to more effective and targeted applications of LLM-based compression.
    % \\

    
    \item {How does the information integrity degrade when recursively compressed by multiple LLM instances?}
    %and what conclusions can be drawn because of it?}

    % The informational integrity of a compression may degrade when compoundingly compressed, potentially leading to information loss or inaccuracies. By analyzing the behavior of compound compression, researchers can identify the limitations and thresholds of LLM-based compression techniques, informing the development of more robust and reliable methods for preserving informational integrity.

\end{enumerate}
